Frobenius structures in star-autonomous categories

It is known that the quantale of sup-preserving maps from a complete lattice to itself is a Frobenius quantale if and only if the lattice is completely distributive. Since completely distributive lattices are the nuclear objects in the autonomous category of complete lattices and sup-preserving maps, we study the above statement in a categorical setting. We introduce the notion of Frobenius structure in an arbitrary autonomous category, generalizing that of Frobenius quantale. We prove that the monoid of endomorphisms of a nuclear object has a Frobenius structure. If the environment category is star-autonomous and has epi-mono factorizations, a variant of this theorem allows to develop an abstract phase semantics and to generalise the previous statement. Conversely, we argue that, in a star-autonomous category where the monoidal unit is a dualizing object, if the monoid of endomorphisms of an object has a Frobenius structure and the monoidal unit embeds into this object as a retract, then the object is nuclear.

==> macrosA.tex <==
\usepackage{xcolor}
\usepackage{tikz}
\usepackage{tikz-cd}
\usepackage{graphbox}

\RequirePackage{amsmath,amssymb,amsfonts}

\RequirePackage{xspace}
\RequirePackage{xcolor}
\RequirePackage{ifthenx}
\RequirePackage{wrapfig}




\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\LS}[2][]{\textcolor{red}{LS #1 : #2}}
\newcommand{\CLL}[2][]{\textcolor{purple}{CLL #1 : #2}}
\newcommand{\AFAIRE}{\red{A FAIRE}}
\newcommand{\RUH}[1][]{\red{#1 Read until here}}


\newcommand{\Myparagraph}[1]{\bigskip\paragraph{\bf #1}}



\newcommand{\trup}[1]{{#1}^{\sharp}}
\newcommand{\Trup}[1]{\trup{(#1)}}
\newcommand{\tr}[1]{\trup{#1}}
\newcommand{\trdown}[1]{{#1}^{\flat}}
\newcommand{\Trdown}[1]{\trdown{(#1)}}
\newcommand{\FUN}{(\,-\,)}
\newcommand{\trupMap}{\trup{\FUN}}
\newcommand{\trdownMap}{\trdown{\FUN}}


\newcommand{\IHom}[1]{[#1]}
\newcommand{\Hom}[1]{\hom(#1)}
\newcommand{\Star}[1]{{#1}^{\ast}}
\newcommand{\STAR}[1]{#1{}^{\ast}}
\newcommand{\SStar}[1]{{#1}\Star{}\Star{}}
\newcommand{\SSStar}[1]{\SStar{#1}{}^{\ast}}
\newcommand{\Perp}[1]{{#1}^{\perp}}
\renewcommand{\Tilde}[1]{\widetilde{#1}}


\newcommand{\HSS}{\IHom{S,S}}

\newcommand{\SI}{\Star{I}}
\newcommand{\SSI}{\SStar{I}}
\newcommand{\SX}{\Star{X}}
\newcommand{\SY}{\Star{Y}}
\newcommand{\SSX}{\SStar{X}}
\newcommand{\SSY}{\SStar{Y}}
\newcommand{\SSSX}{\SSStar{X}}
\newcommand{\SSSY}{\SSStar{Y}}
\newcommand{\HXY}{\IHom{X,Y}}
\newcommand{\HYX}{\IHom{Y,X}}
\newcommand{\HSYSX}{\IHom{\SY,\SX}}
\newcommand{\SM}{\Star{M}}
\newcommand{\SSM}{\Star{M}\Star{}}
\newcommand{\SQ}{\Star{Q}}
\newcommand{\SSQ}{\Star{Q}\Star{}}
\newcommand{\SA}{\Star{A}}
\newcommand{\SSA}{\SStar{A}}
\renewcommand{\SS}{\Star{S}}
\newcommand{\SSS}{\Star{S}\Star{}}
\newcommand{\SB}{\Star{B}}
\newcommand{\SSB}{\SStar{B}}
\newcommand{\SC}{\Star{C}}

\newcommand{\HMM}{\IHom{M,M}}
\newcommand{\HSMSM}{\IHom{\SM,\SM}}

\newcommand{\ev}{ev}
\newcommand{\trace}{tr}

\newcommand{\rto}[1][\qquad]{\xrightarrow{#1}}
\newcommand{\Rto}[1][\qquad]{\xrightarrow{\;\;#1\;\;}}

\newcommand{\eqdef}{:=}
\newcommand{\smallLHS}[2][20mm]{\makebox[#1][l]{${\displaystyle #2}$}}


\newcommand{\tor}{\text{or}}
\newcommand{\Tor}{\;\;\tor\;\;}
\newcommand{\tand}{\text{and}}
\newcommand{\Tand}{\;\;\tand\;\;}
\newcommand{\tiff}{\text{iff}}
\newcommand{\Tiff}{\;\;\tiff\;\;}
\newcommand{\Timplies}{\;\;\text{implies}\;\;}
\newcommand{\Tst}{\;\;\tst\;\;}
\newcommand{\tst}{\text{s.t.}}


\newcommand{\C}{\mathbb{C}}

\newcommand{\homm}[2]{[#1, #2]} 
\newcommand{\ri}{\operatorname{r}}
\newcommand{\li}{\operatorname{l}}




\newcommand{\tensor}{\otimes}
\newcommand{\tesnor}{\otimes}
\newcommand{\cotensor}{\oplus}
\newcommand{\parr}{\rotatebox[origin=c]{180}{$\mathcal{\&}$}}
\newcommand{\comult}{\parr}



\newcommand{\bil}[1][\cdot]{\langle#1\rangle}
\renewcommand{\brack}[1]{\bil[#1]}
\newcommand{\bilr}[1][\cdot]{\bil[#1]{}^{\perp}}
\newcommand{\bill}[1][\cdot]{{}^{\perp}\bil[#1]}


\newcommand{\SLatt}{\ensuremath{\mathsf{SLatt}}\xspace}
\newcommand{\QSets}{\ensuremath{Q\mathsf{Set}}\xspace}
\newcommand{\lrimpl}{\backslash}
\newcommand{\rlimpl}{/}
\newcommand{\rneg}[1][(\,\cdot\,)]{{#1}^{\perp}}
\newcommand{\lneg}[1][(\,\cdot\,)]{{}^{\perp}{#1}}
\newcommand{\Rneg}[1]{{#1}{}^{\perp}}
\newcommand{\Dneg}[1]{\Rneg{#1}\Rneg{}}
\newcommand{\Lneg}[1]{{}^{\perp}{#1}}
\newcommand{\Loplus}{\,{}_{\perp}\!\!\oplus}
\newcommand{\Roplus}{\oplus_{\perp}}

\newcommand{\SLTL}{\SL\tensor L}
\newcommand{\LTSL}{L\tensor \SL}
\newcommand{\SLtL}{\SLTL}
\newcommand{\HLL}{\IHom{L,L}}
\newcommand{\HSLSL}{\IHom{\SL,\SL}}


\newcommand{\myqedhere}[1][0mm]{
  \mbox{
    \begin{tabular}[t]{@{\hspace{0mm}}r@{\hspace{0mm}}}
      \\[#1]
      \qedhere
    \end{tabular}
  }
}

\newcommand{\Fsg}{Frobenius semigroup\xspace}
\newcommand{\iso}{\simeq}
\newcommand{\V}{\ensuremath{\mathcal{V}}}

\newcommand{\Rans}[1]{{#1}^{\vee}}
\newcommand{\Rani}[1]{{#1}^{\wedge}}
\newcommand{\rans}[1]{{#1}{}^{\vee}}
\newcommand{\rani}[1]{{#1}{}^{\wedge}}

\newcommand{\rand}[1]{#1\rani{}\rans{}}
\newcommand{\ranD}[1]{#1\rans{}\rani{}}
\newcommand{\Homs}[1]{{\homm{#1}{#1}}_{\vee}}
\newcommand{\LLs}{{\homm{L}{L}}_{\vee}}
\newcommand{\LLi}{{\homm{L}{L}}_{\wedge}}
\newcommand{\LLst}{\LLs^{t}}
\newcommand{\LLit}{\LLi^{t}}
\newcommand{\LLt}{\LLst}

\newcommand{\mix}{\mathtt{mix}}
\newcommand{\SL}{\Star{L}}
\newcommand{\SSL}{\SStar{L}}
\newcommand{\op}{\operatorname{op}}
\newcommand{\Ld}{{L}^{\op}}
\newcommand{\Md}{{M}^{\op}}
\newcommand{\Qd}{{Q}^{\op}}
\newcommand{\SYTX}{\SY\tensor X}


\newcommand{\ie}{\textit{i.e.}\xspace}
\newcommand{\eg}{\textit{e.g.}\xspace}
\newcommand{\ifff}{\text{  iff  }}
\newcommand{\Ifff}{\quad\text{iff}\quad}
\ifshortversion
\renewcommand{\st}{\text{  s.t.  }}
\else
\newcommand{\st}{\text{  s.t.  }}
\fi
\newcommand{\contr}{a contradiction\xspace}
\newcommand{\Impl}[2]{(#1) $\Rightarrow$ (#2)}
\newcommand{\ra}{right-adjoint\xspace}
\newcommand{\la}{left-adjoint\xspace}
\newcommand{\jp}{sup-preserving\xspace}
\renewcommand{\mp}{inf-preserving\xspace}
\newcommand{\LL}{L^{L}}

\newcommand{\fun}{(-)}
\newcommand{\adj}{\dashv}
\newcommand{\rightIso}[1]{\xrightarrow{\,\overset{\raisebox{4pt}{{$\scriptsize
          #1$}}}{\raisebox{-4pt}{$\tiny \sim$}}\,}}
\newcommand{\rIso}[1]{\rightIso{#1}}

\newcommand{\bm}{bracketed magma\xspace}
\newcommand{\abm}{associative bracketed magma\xspace}
\newcommand{\id}{\mathtt{id}}

\newcommand{\lact}[1][A]{\alpha^{\ell}_{#1}}
\newcommand{\ract}[1][B]{\alpha^{\rho}_{#1}}
\newcommand{\affine}{affine\xspace}
\newcommand{\pseudoaffine}{pseudo-affine\xspace}
\newcommand{\paffine}{\pseudoaffine}


\newcounter{useDiagCount}
\setcounter{useDiagCount}{0}
\newcommand{\useDiagram}[2][]{
  \ifthenelse{\isinteger{#1}}{
    \setcounter{useDiagCount}{#1}
    \includegraphics[page=#1,align=c]{#2}
  }{
    \stepcounter{useDiagCount}
    \def\page{\theuseDiagCount}
    \includegraphics[page=\page,align=c,#1]{#2}
  }
}

\newcommand{\cl}{complete lattice\xspace}
\newcommand{\cd}{completely distributive\xspace}
\newcommand{\cdlatt}{\cd lattice\xspace}
\newcommand{\upTensor}{\widehat{\tensor}}
\newcommand{\RT}{Raney's theorem\xspace}

\newcommand{\set}[1]{\{ \,#1\,\}}
\newcommand{\downset}[1]{\downarrow #1}
\newcommand{\two}{\mathbf{2}}
\newcommand{\closure}[1]{\overline{#1}}
\newcommand{\positive}{positive\xspace}
\newcommand{\strong}{strongly continuous\xspace}

\newcommand{\card}[1]{|#1|}

\newcommand{\leftA}{l}
\newcommand{\rightA}{r}
\newcommand{\leftB}{\leftA^{-1}}
\newcommand{\rightB}{\rightA^{-1}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\pairing}[1]{\langle#1\rangle}
\newcommand{\Pairing}[1]{(#1)}
\newcommand{\innerH}[1]{\pairing{#1}_{H}}
\newcommand{\normH}[1]{||#1||_{H}}

\newcommand{\qmult}{\ast}
\newcommand{\Cstar}{\ensuremath{\mathrm{C}^{\ast}}}

\newcommand{\saut}{$\ast$-autonomous\xspace}
\newcommand{\sautcat}{\saut category\xspace}
\newcommand{\sautcats}{\saut categories\xspace}
\newcommand{\autcat}{autonomous category\xspace}
\newcommand{\autcats}{autonomous categories\xspace}
\newcommand{\smcc}{symmetric monoidal closed category\xspace}
\newcommand{\smccs}{symmetric monoidal closed categories\xspace}
\newcommand{\chu}{\operatorname{Chu}_{\V,\zero}}
\newcommand{\Pair}{\operatorname{Pair}_{\V,\zero}}
\newcommand{\Ens}{\mathbf{Set}}
\newcommand{\sem}[1]{{\textbf{Sem}}_{#1}}
\newcommand{\vect}{\textbf{Vect}}


\newcommand{\radj}[1]{\rho(#1)}
\newcommand{\ladj}[1]{\ell(#1)}
\newcommand{\supj}{\mbox{$\bigvee_j$}}
\newcommand{\cotight}{cotight\xspace}


\newcommand{\pr}[1]{\operatorname{pr}_{#1}}


\newcommand{\zero}{I}
\newcommand{\SATA}{\SA\tensor A}
\newcommand{\ATSA}{A\tensor \SA}
\newcommand{\HAA}{\IHom{A,A}}
\newcommand{\frob}{(A,B,\epsilon,\mu_A, \leftA,\rightA)}




\newcommand{\G}{\SATA}

\newcommand{\D}{\HAA}

\newcommand{\norm}[1]{\left\lVert #1\right\rVert}



==> theorems.tex <==
\RequirePackage{amsthm}

\ifshortversion
\theoremstyle{definition}
\newtheorem{fact}[theorem]{Fact}
\else
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{notation}{Notation}

\theoremstyle{remark}
\newtheorem{remark}{Remark}
\newtheorem{conjecture}{Conjecture}
\newtheorem{claim}{Claim}
\newtheoremstyle{exmpl}
{3pt}
{3pt}
{}
{}
{\bf}
{.}
{.5em}
{\thmname{#1}\thmnumber{ #2}\thmnote{: {\bf #3}}}

\theoremstyle{exmpl}
\newtheorem{example}[theorem]{Example}
\newcommand{\qedExample}{\hfill$\Diamond$}
\RequirePackage{ifthen}
\newenvironment{Example}[1][]{\bigskip\ifthenelse{\equal{#1}{}}{\begin{example}}{\begin{example}[#1]}}{\qedExample\end{example}}
\fi



\providecommand*\theoremautorefname{statement}
\providecommand*\factautorefname{Fact}


\theoremstyle{plain}

\newtheorem*{theorem*}{Theorem}
\newcounter{thm}
\renewcommand{\thethm}{\Alph{thm}}
\newtheorem{thmIntro}[thm]{Theorem}

\theoremstyle{definition}
\newtheorem*{definition*}{Definition}



